RETAIN: An Interpretable Predictive Model for Healthcare using Reverse Time Attention Mechanism

Accuracy and interpretability are two dominant features of successful predictive models. Typically, a choice must be made in favor of complex black box models such as recurrent neural networks (RNN) for accuracy versus less accurate but more interpretable traditional models such as logistic regression. This tradeoff poses challenges in medicine where both accuracy and interpretability are important. We addressed this challenge by developing the REverse Time AttentIoN model (RETAIN) for application to Electronic Health Records (EHR) data. RETAIN achieves high accuracy while remaining clinically interpretable and is based on a two-level neural attention model that detects influential past visits and significant clinical variables within those visits (e.g. key diagnoses). RETAIN mimics physician practice by attending the EHR data in a reverse time order so that recent clinical visits are likely to receive higher attention. RETAIN was tested on a large health system EHR dataset with 14 million visits completed by 263K patients over an 8 year period and demonstrated predictive accuracy and computational scalability comparable to state-of-the-art methods such as RNN, and ease of interpretability comparable to traditional models.

==> data_stat.tex <==
\begin{table}[t]
\caption{Statistics of Sutter PAMF dataset}
\label{table:data_stat}
% \small
\vspace*{-2mm}
\centering
\begin{tabular}{l|c}
\textbf{Dataset} & \textbf{Sutter PAMF}\\
\hline
\hline
\# of patients & 263,683\\ 
\# of visits & 14,366,030\\
Avg. \# of visits per patient & 54.5\\
\hline
\# of unique medical codes & 615\\
- \# of unique diagnosis codes & 283\\
- \# of unique medication codes & 94\\
- \# of unique procedure codes & 238\\
\hline
Avg. \# of codes per visit & 7.88\\
\hline
Max \# of codes per visit & 440\\
\hline
\begin{tabular}{@{}l@{}}
(95\%, 99\%) percentile\\ \# of codes per visit
\end{tabular}
& (22, 53)\\
\hline
\end{tabular}
\vspace{-0.1in}
\end{table}

==> hf_codes.tex <==
\begin{table}[t]
\centering
    \caption{Qualifying ICD-9 codes for heart failure}
    \begin{tabular}{|l|c|}
    \hline
    ICD-9 Code & Description \\
    \hline \hline
    398.1 & Rheumatic heart failure (congestive) \\
    \hline
    402.01 & Rheumatic heart failure (congestive) \\
    \hline
    398.1 & Rheumatic heart failure (congestive) \\
    \hline    
    \end{tabular}
\label{tab:hfResult}
\end{table} 

==> hf_data.tex <==
\begin{table}
\caption{Basic statistics of the Sutter Health heart failure dataset. (D:Diagnosis code, R:Medication code, P:Procedure code)}
\label{table:data}
\centering
\begin{tabular}{l|c||l|c}
\# of cases & 3,884 & \# of controls & 28,903 \\
\hline
\# of visits & 14,366,030 & Max \# of codes in a visit & 62 \\
\hline
Avg. \# of visits per patient & 54.48 & Avg. \# of Dx codes in a visit & 1.83\\
\hline
\# of unique medical codes & 615 (D:283, R:94, P:238) & Max \# of Dx codes in a visit & 42 \\
\end{tabular}
\end{table}

==> interpretationOld.tex <==
In this section, we describe how to interpret the prediction made by \alg. When we are predicting the diagnosis codes $Y_T$ given $X_1, X_2, \ldots, X_T$, we can generate $\alpha_1, \ldots, \alpha_T$ and $\bm{\beta}_1, \ldots, \bm{\beta}_T$'s by Eq~\eqref{eq:alpha} and Eq~\eqref{eq:beta}. 

Interpreting the $\alpha$'s is straightforward since they represent each visit's contribution in making the prediction $\widehat{\yb}_{T}$. The $\alpha$'s are specifically generated using the Softmax function to facilitate intuitive interpretation.\footnote{The same approach was suggested by Bahdanau et al.\cite{bahdanau2014neural}.} 

Interpreting the $\bm{\beta}$'s is a little trickier than interpreting the $\alpha$'s since each $\bm{\beta}_t$ is applied to the visit embedding $\vb_t \in \mathbb{R}_+^m$, which is a non-negative real-valued vector. Here we propose a simple and logical method to obtain the code-level interpretation. Our method is based on the coordinate-wise analysis of the visit embedding $\vb_t$. Given a visit $X_t = \{c_1, c_2, \ldots, c_n\}$, the visit embedding $\vb_t$ can be viewed as follows,
\begin{equation}
\vb_t = \sum_{i=1}^{n} \Wb_{emb}[:,i]
\end{equation}
where $\Wb_{emb}[:,i] \in \mathbb{R}_{+}^{m}$ can be viewed as the non-negative representation\footnote{We use the MATLAB notation to represent a column of a matrix} of the medical code $c_i \in \mathcal{C}$. Therefore, the prediction contribution of the $j$-th coordinate of the visit embedding $\vb_t$ can be expressed as follows,
\begin{equation}
\mbox{contribution of }\vb_t^{(j)} = \sum_{i=1}^{n} \bm{\beta}_{t}^{(j)} \Wb_{emb}[:,i]^{(j)} \label{eq:visit_contribution}
\end{equation}
Eq~\eqref{eq:visit_contribution} shows us that we can decompose the prediction contribution of the $j$-th coordinate of $\vb_t$ into the $j$-th coordinate of each medical code representation $\Wb_{emb}[:,1]^{(j)}, \ldots, \Wb_{emb}[:,n]^{(j)}$. Generalizing this to all coordinates of the visit $\vb_t \in \mathbb{R}^{m}$, we can determine the prediction contribution of each medical code $c_i \in X_t$ as follows,
\begin{equation}
f_c(c_i \in \xb_t) = \sum_{j=1}^{m} \bm{\beta}_{t}^{(j)} \Wb_{emb}[:,i]^{(j)} = \bm{\beta}_{t}^{\top} \Wb_{emb}[:,i]
\end{equation}
where we use $f_c$ to denote the function for calculating the contribution of a medical code. Therefore, in order to calculate the contribution of a medical code $c_i \in X_t$ in making the prediction $\widehat{\yb}_{T}$, we can use a simple inner-product between the code-level attention vector $\bm{\beta}_t$ and the medical code representation $\Wb_{emb}[:,i]$. 

This simple code-level interpretation is possible because we are using non-negative values for both the embedding matrix $W_{emb}$ and the code-level attention vector $\bm{\beta}$, so we can avoid considering how to deal with negative values.

Note that the prediction contribution $f_c(c_i \in X_t)$ should be understood as a relative value that should be compared with the prediction contributions of other medical codes in the same visit $X_t$. The prediction contribution of the visit $X_t$ itself is adjusted by $\alpha_t$. Therefore, when comparing prediction contributions of medical codes from different visits, we must take into account the visit-level attention scalar $\alpha$'s.

==> introOld.tex <==

The adoption of Electronic Health Records (EHR) by large hospitals has opened the possibility of applying statistical methods to improve the quality of clinical services. Medical prognosis is a practice of forecasting the course of a disease, which is a very important aspect of medical care. Accurate prognosis can facilitate timely intervention and more aggressive treatment, which can not only save human lives but also cut down the problematic healthcare cost we are facing. \tbedit{Stronger, citations for applications.}

Many recent works utilizing the EHRs tried to make some form of prediction by studying the past records of patients: predicting the stage of Parkinson's disease \cite{hammerla2015pd}, chronic obstructive pulmonary disease \cite{wang2014unsupervised}, Alzheimer's disease \cite{sukkar2012disease,zhou2013modeling}, interstitial lung disease \cite{schulam2015framework}. \tbedit{Broader review, big picture ideas, based on \cite{mould2012models}.}

In this work we do not focus on predicting the course of a single disease, but rather attempt to forecast the course of a patient's medical status over time. This approach will take into account the hidden relationships among various diseases and make comprehensive forecast of the patient status in the future. \tbedit{Not an effective paragraph.}

Recently there have been a few studies that applied deep learning methods to perform such comprehensive prediction task. Lipton et al. \cite{lipton2015learning} used Recurrent Neural Network (RNN) to classify 128 diagnoses using data collected from ICU patients. Choi et al. \cite{choi2015doctor} used RNN to predict the diseases and medications likely to occur in the patient's next visit. However, while RNN excels at making predictions for sequence data, it is difficult to interpret its inner-working. \tbedit{Be careful about positioning here: RNNs might not be the very best, at least be careful about it.}

Interpretability is a vital element in healthcare applications \cite{caruana2015intelligible}. The objective of many machine learning based healthcare applications is to assist physicians make informed decision, which cannot be achieved without interpretable models. There are three schools of interpretation: \tbedit{Expand.}

In this work, we propose \alg, a novel attention based prognosis model that provides detailed interpretation of the prediction results while demonstrating the performance comparable to the state-of-the-art machine learning models.
When making a prediction by looking at the patient's past visits, \alg not only explains which past visit is most influential, but also tells how much each medical code (\textit{e.g.} diagnosis code, medication code, procedure code) in that visit contributed to making the prediction. 
This is made possible by our novel attention mechanism inspired by the behavior of human physicians. 
The key idea of our model is shown in Figure \ref{fig:idea}, with comparison to other popular models. \tbedit{Describe the idea in more details.}

In the following section, we discuss the related work focusing on predictive healthcare applications, and recently developed attention models. In section three, we provide detailed explanation of our model, and its interpretation algorithm. In section four, we demonstrate the state-of-the-art predictive performance of \alg and provide examples of clinical interpretations. We conclude our work in section five.

\begin{figure}[t]
\centering
\includegraphics[scale=0.44]{./figs/diff2}
\caption{We describe a scenario where we try to predict \textit{eye disorder} and \textit{hypertension} given two visit records. The numbers in the parentheses indicate the attention values. (a) Using basic RNN does not offer any interpretation. (b) Applying the basic attention mechanism to the RNN allows us to analyze the visit-level influence. (c) \alg offers full interpretation where we can analyze both the visit-level influence and the code-level influence.\tbedit{Too small.} }
\label{fig:idea}
\end{figure}

==> old_intro.tex <==
\textbf{Outline}
\begin{enumerate}
\item \textbf{Medical prognosis using EHR data}:
\begin{itemize}
\item Importance, possibility  (similar to Dr. AI)
\item Review of recent advances
\end{itemize} 
\item \textbf{Interpretable models in healthcare}:
\begin{itemize}
\item Motivation: the need for such models: \cite{caruana2015intelligible}
\item Lack of interpretability in sophisticated machine learning models.
\end{itemize}
\item \textbf{Approaches for interpretability}
\begin{itemize}
\item Three schools + ref
\end{itemize}
\item \textbf{Outline of the ideas}:
\begin{itemize}
\item Without loss of generality, we focus on disease progression modeling.
\item Our goal: preserve performance of RNN, but make it interpretable.
\item Key idea:  Attention models
\item But with key modification
\item Additional sparsity etc
\end{itemize}
\item \textbf{List of advantages of our model}: 
\begin{enumerate}
\item Interpretability: easier to interpret than even the state-space models
\item Embedding: better embedding than \verb+Med2Vec+ and Skip-thought (?)
\item Retain advantages of attention models: longer memory.
\item Seq2seq modeling advantages
\end{enumerate}
\item \textbf{Experiments}
\begin{itemize}
\item Accuracy evaluation
\item Interpretability evaluation
\end{itemize}
\end{enumerate}

==> old_method.tex <==

\begin{equation}
\eb_i = \mathrm{RNN}(\vb_{1:i}, \yb_{1:i}),
\end{equation}

Using these powerful representations, \alg generates the attention sequence vectors for each visit as follows: 
\begin{equation}
\ab_{1:i}^{(i)} = \mathrm{MLP}(\eb_{i}),
\label{eq:attention}
\end{equation}

\alg generates the patient representation at each visit as follows

\noindent where $\odot$ denotes element-wise product of two vectors. The final prediction is generated as follows:
\begin{equation}
\widehat{\yb}_i = \mathrm{softmax}(\Wb\pb_i),
\end{equation}

\paragraph{Computational simplification}
The general form of attention mechanism in Eq. \eqref{eq:attention} can be computationally expensive.  We propose a simplification as follows. \tbedit{Update this.}

==> related.tex <==
In this section, we overview popular classes of machine learning algorithms and the extent of interpretability of them. While researchers always attempt to get insights into what their proposed approach learn, the degree of intelligibility of the methods differ: simpler models such as linear regression, decision trees, nearest neighbors are easier to interpret compared to neural networks, boosted models, and kernel methods \cite{caruana2015intelligible}.

% \textbf{Predictive Analysis in Healthcare.} Predicting the progression of a specific disease has been the focus of many clinical applications. Studies from the medical field such as modeling the progression of chronic kidney disease to kidney failure\cite{tangri2011predictive}, the progression of Alzheimer's disease\cite{ito2010disease} or type 2 Diabetes\cite{de2006mechanism} focus on a single disease, requiring expert medical knowledge.

% Recently, many researchers applied data driven methods to EHR datasets for disease progression modeling. 
% Majority of them focus on a specific disease such as Parkinson's disease\cite{hammerla2015pd}, Alzheimer's disease\cite{sukkar2012disease,zhou2012modeling,zhou2013modeling}, interstitial lung disease\cite{schulam2015framework}, glaucoma\cite{liu2013longitudinal} or chronic obstructive pulmonary disease\cite{wang2014unsupervised}.
% The studies above not only focus on a single disease, but they also have not been tested on large datasets consisting of hundreds of thousands of patients and millions of visits.

% There have been a few studies making predictions for multiples diseases. Leiva-Murillo et al.\cite{leiva2011visualization} used continuous-time Hidden Markov Model (HMM) to capture the progression of various mental disorders. 
% HMM models, however, are limited by the Markov assumption. 
% Choi et al.\cite{choi2015constructing} used Hawkes process to capture the hidden relationships among various diseases and predict the future risk.
% Hawkes process, however, assumes a linear interaction among different event types (diseases), which is unsuitable for modeling the complex nature of disease progression. 
% %(Hawkes process also has scalability issues since the its training time increases quadratically by the number of events in the input sequence?)
% Lipton et al.\cite{lipton2015learning} used RNN to predict the diagnosis of 128 diseases given the real-valued lab results of ICU patients. Choi et al.\cite{choi2015doctor} used RNN to predict the future diagnosis codes, medication codes and the visit time using the longitudinal visit records. However, while RNN shows impressive prediction performance for sequence data, it is difficult to explain how the past inputs influenced the outcomes. In this work, we utilize both feedforward network and RNN to utilize the power of representation learning while providing transparent interpretation. 
